GC-Bench: An Open and Unified Benchmark for Graph Condensation

Graph condensation (GC) has recently garnered considerable attention due to its ability to reduce large-scale graph datasets while preserving their essential properties. The core concept of GC is to create a smaller, more manageable graph that retains the characteristics of the original graph. Despite the proliferation of graph condensation methods developed in recent years, there is no comprehensive evaluation and in-depth analysis, which creates a great obstacle to understanding the progress in this field. To fill this gap, we develop a comprehensive Graph Condensation Benchmark (GC-Bench) to analyze the performance of graph condensation in different scenarios systematically. Specifically, GC-Bench systematically investigates the characteristics of graph condensation in terms of the following dimensions: effectiveness, transferability, and complexity. We comprehensively evaluate 12 state-of-the-art graph condensation algorithms in node-level and graph-level tasks and analyze their performance in 12 diverse graph datasets. Further, we have developed an easy-to-use library for training and evaluating different GC methods to facilitate reproducible research. The GC-Bench library is available at https://github.com/RingBDStack/GC-Bench.

==> 2_problem_formulation.tex <==
\section{Preliminary and Problem Formulation}
% \section{Problem Formulation}
\label{sec:problem}
% We formulate the graph condensation problem into two categories: node-level condensation and graph-level condensation.
% 
% \paragraph{Notations}
Let $\mathcal{G}=\{\mathbf{X}, \mathbf{A}\}$ be a graph, where $\mathbf{X}\in\mathbb{R}^{N\times d}$ is the node feature matrix of $N$ nodes with $d$-dimension features and $\mathbf{A}\in\mathbb{R}^{N\times N}$ is the adjacency matrix. 
% $\mathcal{V}$ is the node set with $N$ nodes, $\mathcal{E}$ is the edge set, , . 
% Typically, a graph learning model can be parameterized as $f: (\mathbf{X},\mathbf{A})\rightarrow \mathbb{R}^{N\times d}$, which learns a $d$-dimensional embedding vector for each node.
The goal of \textbf{Graph Condensation} is to achieve comparable results on synthetic condensed graph dataset $\mathbf{G}'$ as training on the original graph dataset $\mathbf{G}$. 
The general framework of GC is shown in Figure~\ref{fig:framework}. 
In general, the objective of GC can be summarized as the following formula: 
\begin{equation}
    \mathbf{G}'={\arg\min}_{\mathbf{G}'}\mathcal{L}(f_{\theta_{\mathbf{G}'}}(\mathbf{G}),f_{\theta_{\mathbf{G}}}(\mathbf{G})),  
\end{equation}
where $f_{\theta_{\mathbf{G}'}}$ and $f_{\theta_{\mathbf{G}}}$ denote the graph learning model trained on $\mathbf{G}'$ and $\mathbf{G}$, and $\mathcal{L}$ denotes the loss function that measures the difference of these two models. 
For \textbf{Node-level Condensation}, the original dataset $\mathbf{G}=\{\mathcal{G}\}=\{\mathbf{X}\in\mathbb{R}^{N\times d}, \mathbf{A}\in\mathbb{R}^{N\times N}\}$ and the condensed dataset $\mathbf{G}'=\{\mathcal{G}'\}=\{\mathbf{X}\in\mathbb{R}^{N'\times d'}, \mathbf{A}\in\mathbb{R}^{N'\times N'}\}$, where $N'\ll N$. 

For \textbf{Graph-level Condensation}, the original dataset $\mathbf{G}=\{\mathcal{G}_1, \mathcal{G}_2, \cdots, \mathcal{G}_n\}$ and the condensed dataset $\mathbf{G}'=\{\mathcal{G}'_1, \mathcal{G}'_2, \cdots, \mathcal{G}'_{n'}\}$, where $n'\ll n$. 


% \paragraph{Node-level Condensation}
% Given a graph $G$ with the labeled node set $\mathcal{V}_L$ and their labels $\mathbf{Y}_L \in \mathbb{R}^C$, where each node $v_i$ is associated with a label $\mathbf{y}_i$. 
% Node-level condensation aims to 
% % train a node classifier $f_{\boldsymbol{\theta}}:v \mapsto \mathbb{R}^C$ to predict the labels $\mathbf{Y}_U$ of the remaining nodes $\mathcal{V}_U = \mathcal{V} \setminus \mathcal{V}_L$.

% \paragraph{Graph-level Condensation}
% Denote $\mathbf{G}$ as the graph set. 
% Given the labeled graph set $\mathbf{G}_L$ and their labels $\mathbf{Y}_L \in \mathbb{R}^C$, where each graph $\mathcal{G}_i$ is associated with a label $\mathbf{y}_i$. 
% Graph-level condensation task aims to 
% train a graph classifier $\mathcal{F}_{\boldsymbol{\theta}}:\mathcal{G} \mapsto \mathbb{R}^C$ to predict the labels $\mathbf{Y}_U$ of the unlabeled graphs $\mathbf{G}_U = \mathbf{G} \setminus \mathbf{G}_L$. 

==> 2_related_work.tex <==
\section{Related Works}
\label{sec:related_works}
\zytodo{a brief summary of related works, Table}
\subsection{Dataset Distillation}

\subsubsection{Coreset selection methods}
In the context of dataset condensation, coreset selection methods are instrumental in identifying representative nodes from the original dataset to induce a subgraph from the selected nodes. Since our main focus is on dataset synthesis methods, this section delineates three primary coreset methods. 

\textbf{Random} For random selection baseline, a fixed number of nodes are selected randomly from the original graph. 

\textbf{Herding} Originally applied in continual learning scenarios\cite{Rebuffi_Kolesnikov_Sperl_Lampert_2017}\cite{Castro_Marín-Jiménez_Guil_Schmid_Alahari_2018}, this method selects samples that approximate the cluster center, effectively capturing the centroid of data distributions. 

\textbf{K-Center} This method, as detailed by \cite{Farahani_Hekmatfar_2009} and \cite{Sener_Savarese_2017}, optimizes the selection of central nodes to minimize the maximum distance between any node and its nearest cluster center.

\subsection{Graph Condensation}
The substantial memory and computational demands of training graph neural networks on large-scale graph datasets necessitate the invention of Graph Condensation (GC). GC is designed to transform extensive graph datasets into condensed, smaller-scale synthetic datasets that allow neural networks to achieve performance comparable to training on full datasets.

\textbf{GM-Graph Condensation with Gradient Matching} This method focuses on generating synthetic graph datasets that optimize the training process for Graph Neural Networks (GNNs). It employs a gradient matching technique to minimize the loss on both the synthetic and original graphs. 

\cite{Jin_Zhao_Zhang_Liu_Tang_Shah_2021} introduced GCond, the first graph condensation method based on gradient-matching, which aligns the model gradients between models trained on full and synthetic datasets. GCond's bi-level optimization adds considerable computational complexity, making it resource-intensive for large-scale graph condensation tasks. To address this, \cite{Jin_Tang_Jiang_Li_Zhang_Tang_Yin_2022} developed DosCond, utilizing a one-step gradient matching scheme which only matches the gradients for the model initialization $\theta_0$ and uses a probabilistic model to model graph structure for graph classification. For better structural preservation, \cite{yang2023does} proposed a scheme SGDD by converting the adjacency matrix into Laplacian Energy Distribution and broadcasting the original matrix to the generation of synthetic datasets, which significantly improved the cross-architecture performance of synthetic datasets.

\textbf{TM-Graph Condensation with Trajectory Matching} The Trajectory-matching method matches their long-term GNN training trajectories under the guidance of offline expert trajectories which are obtained from models trained on original datasets. 


\cite{Zheng_Zhang_Chen_Nguyen_Zhu_Pan_2023} developed the first graph condensation method based on trajectory-matching, which synthesizes a graph node-set as graph-free data using trajectory meta-matching scheme and evaluates the quality of condensed data using graph neural tangent kernel(GNTK) ridge regression. Subsequently, \cite{DBLP:journals/corr/abs-2402-05011} critiqued the potentially biased and restricted supervision signals derived from the original graph when optimizing synthetic datasets in SFGC. To address these issues, they proposed the GEOM method, which employs a curriculum learning strategy to train expert trajectories, which are aligned using an expanding window matching technique. Inspired by Knowledge Distillation, GEOM also integrates information extraction of teacher models.


% \subsection{Existing Benchmarks}

==> table/GCondenser.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Comparison of GCondenser and \modelname}
\label{tab:gcondenser}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{cclll}
\hline
\multicolumn{3}{c}{\textbf{Benchmark Coverage}} &
  \textbf{GCondenser} &
  \textbf{GC-Bench (Ours)} \\ \hline
 &
  \multicolumn{2}{c}{Traditional  Methods} &
  Random, K-Center &
  \begin{tabular}[c]{@{}l@{}}Random, K-Center,  Herding\end{tabular} \\
 &
  \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}Gradient  Matching} &
  \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}GCond, DosCond, SGDD\end{tabular} &
  \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}GCond, DosCond, SGDD\end{tabular} \\
 &
  \multicolumn{2}{c}{Distribution Matching} &
  GCDM, DM & GCDM, DM
   \\
 &
  \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}Trajectory Matching} &
  \cellcolor[HTML]{EFEFEF}SFGC &
  \cellcolor[HTML]{EFEFEF}SFGC, GEOM \\
 &
  \multicolumn{2}{c}{KRR} &
  — &
  KiDD \\
\multirow{-6}{*}{\rotatebox[origin=c]{90}{\textbf{Algorithm}}} &
  \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}CTC} &
  \cellcolor[HTML]{EFEFEF}— &
  \cellcolor[HTML]{EFEFEF}Mirage \\ \hline
 &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Node-level\\ Homogenerous\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}\cora, \citeseer, \arxiv\\ \flickr, \reddit, \textit{PubMed}\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}\cora, \citeseer, \arxiv\\ \flickr, \reddit\end{tabular} \\
 &
  \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}Node-level\\ Heterogeneous\end{tabular}} &
  \cellcolor[HTML]{EFEFEF}— &
  \cellcolor[HTML]{EFEFEF}\acm, \dblp \\
\multirow{-5}{*}{\rotatebox[origin=c]{90}{\textbf{Datasets}}} &
  \multicolumn{2}{c}{Graph-level} &
  — &
  \begin{tabular}[c]{@{}l@{}}\nci, \dd, \bace\\ \bbbp, \hiv\end{tabular} \\ \hline
 &
  \multicolumn{2}{c}{\cellcolor[HTML]{EFEFEF}Nodel-level} &
  \cellcolor[HTML]{EFEFEF}node classification &
  \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}node classification\\ link prediction\\ anomaly detection\end{tabular} \\
\multirow{-4}{*}{\rotatebox[origin=c]{90}{\textbf{Tasks}}} &
  \multicolumn{2}{c}{Graph-level} &
  — &
  graph classification \\ \hline
 &
   &
  \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Condensation\\ Ratios\end{tabular} &
  \cellcolor[HTML]{EFEFEF}\checkmark &
  \cellcolor[HTML]{EFEFEF}\checkmark \\
 &
   &
  \begin{tabular}[c]{@{}l@{}}Impact of\\ Struture\end{tabular} &
  structure v.s. structure-free &
  \makecell[l]{structure v.s. structure-free\\structure properties \\
  (homogeneity and heterogeneity,\\ homophily and heterophily)} \\
 &
  \multirow{-4}{*}{Perf.} &
  \cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Impact of\\ Initialization\end{tabular} &
  \cellcolor[HTML]{EFEFEF}\checkmark &
  \cellcolor[HTML]{EFEFEF}\checkmark \\ \cline{2-5} 
 &
   &
  Backbone Gen. &
   & \makecell[l]{
  GNN: \textit{SGC}, \textit{GCN}, \textit{GraphSAGE}\\\textit{APPNP}, \textit{ChebyNet}\\
  non-GNN: \textit{MLP}, \textit{Graph Transformer}} 
   \\
 &
   &
  \cellcolor[HTML]{EFEFEF}Backbone Trans. &
  \cellcolor[HTML]{EFEFEF}\makecell[l]{\textit{SGC} and \textit{GCN} transfer to\\\textit{SGC}, \textit{GCN}, \textit{GraphSAGE}\\\textit{APPNP}, \textit{ChebyNet}, \textit{MLP}} &
  \cellcolor[HTML]{EFEFEF}All combinations of backbone models \\
 &
   &
  Task Gen. &
  — &
  \checkmark \\
 &
  \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Gen.\\ and\\ Trans.\end{tabular}} &
  \cellcolor[HTML]{EFEFEF}Task  Trans. &
  \cellcolor[HTML]{EFEFEF}— &
  \cellcolor[HTML]{EFEFEF}\checkmark \\ \cline{2-5} 
 &
   &
  Time &
  \checkmark &
  \checkmark \\
\multirow{-15}{*}{\rotatebox[origin=c]{90}{\textbf{Evaluation Dimensions}}} &
  \multirow{-2}{*}{Efficiency} &
  \cellcolor[HTML]{EFEFEF}Space &
  \cellcolor[HTML]{EFEFEF}— &
  \cellcolor[HTML]{EFEFEF}\checkmark \\ \hline
\end{tabular}
}
\end{table}

==> table/Tasks.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{NClu}}    & \multicolumn{1}{c|}{\multirow{2}{*}{Ratio(r)}} & \multicolumn{4}{c|}{Citeseer}                                                                                 & \multicolumn{1}{c|}{\multirow{2}{*}{Ratio(r)}} & \multicolumn{4}{c}{Cora}                                                                  \\ \cmidrule(lr){3-6} \cmidrule(l){8-11} 
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{}                          & ACC                  & NMI                  & ARI                  & \multicolumn{1}{c|}{F1}                  & \multicolumn{1}{c|}{}                          & ACC                  & NMI                  & ARI                  & F1                   \\ \midrule
\multicolumn{1}{l|}{K-means}                  & \multicolumn{1}{c|}{\multirow{7}{*}{Full}}     & 54.4                 & 31.2                 & 28.5                 & \multicolumn{1}{c|}{41.3}                & \multicolumn{1}{c|}{\multirow{7}{*}{Full}}     & 50.0                 & 31.7                 & 37.6                 & 23.9                 \\
\multicolumn{1}{l|}{VGAE}                     & \multicolumn{1}{c|}{}                          & 39.2                 & 16.3                 & 10.1                 & \multicolumn{1}{c|}{27.8}                & \multicolumn{1}{c|}{}                          & 59.2                 & 40.8                 & 45.6                 & 34.7                 \\
\multicolumn{1}{l|}{ARGA}                     & \multicolumn{1}{c|}{}                          & 57.3                 & 35.0                 & 34.1                 & \multicolumn{1}{c|}{54.6}                & \multicolumn{1}{c|}{}                          & 64.0                 & 44.9                 & 61.9                 & 35.2                 \\
\multicolumn{1}{l|}{MGAE}                     & \multicolumn{1}{c|}{}                          & 66.9                 & {\ul 41.6}           & {\ul 42.5}           & \multicolumn{1}{c|}{52.6}                & \multicolumn{1}{c|}{}                          & 68.1                 & 48.9                 & 53.1                 & \textbf{56.5}        \\
\multicolumn{1}{l|}{AGC}                      & \multicolumn{1}{c|}{}                          & 67.0                 & 41.1                 & 41.5                 & \multicolumn{1}{c|}{\textbf{62.5}}       & \multicolumn{1}{c|}{}                          & 68.9                 & {\ul 53.7}           & {\ul 65.6}           & 44.8                 \\
\multicolumn{1}{l|}{DAEGC}                    & \multicolumn{1}{c|}{}                          & {\ul 67.2}           & 39.7                 & 41.0                 & \multicolumn{1}{c|}{{\ul \textbf{63.6}}} & \multicolumn{1}{c|}{}                          & 70.4                 & 52.8                 & \textbf{68.2}        & 49.6                 \\
\multicolumn{1}{l|}{SUBLIME}                  & \multicolumn{1}{c|}{}                          & \textbf{68.5}        & \textbf{44.1}        & \textbf{43.9}        & \multicolumn{1}{c|}{{\ul 63.2}}          & \multicolumn{1}{c|}{}                          & \textbf{71.3}        & \textbf{54.2}        & 63.5                 & {\ul 50.3}           \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{GCond}}   & \multicolumn{1}{c|}{1.30\%}                    & 61.8                 & 34.0                 & 34.7                 & \multicolumn{1}{c|}{55.9}                & \multicolumn{1}{c|}{0.90\%}                    & 46.6                 & 36.7                 & 27.3                 & 41.2                 \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{2.60\%}                    & 59.6                 & 33.0                 & 32.6                 & \multicolumn{1}{c|}{\textbf{50.3}}       & \multicolumn{1}{c|}{1.80\%}                    & 49.9                 & 39.3                 & 27.9                 & 44.3                 \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{5.20\%}                    & 57.8                 & 32.0                 & 30.2                 & \multicolumn{1}{c|}{{\ul 54.8}}          & \multicolumn{1}{c|}{3.60\%}                    & 44.6                 & 40.9                 & 25.1                 & 37.3                 \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{DosCond}} & \multicolumn{1}{c|}{1.30\%}                    & 28.6                 & 10.2                 & 6.3                  & \multicolumn{1}{c|}{25.1}                & \multicolumn{1}{c|}{0.90\%}                    & 30.2                 & 0.4                  & 0.0                  & 6.8                  \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{2.60\%}                    & 57.1                 & 31.4                 & 26.2                 & \multicolumn{1}{c|}{49.5}                & \multicolumn{1}{c|}{1.80\%}                    & 30.2                 & 0.4                  & 0.0                  & 6.8                  \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{5.20\%}                    & 44.3                 & 20.6                 & 17.0                 & \multicolumn{1}{c|}{38.6}                & \multicolumn{1}{c|}{3.60\%}                    & 29.6                 & 16.2                 & 7.7                  & 23.4                 \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{SGDD}}    & \multicolumn{1}{c|}{1.30\%}                    & 56.5                 & 27.3                 & 26.8                 & \multicolumn{1}{c|}{50.6}                & \multicolumn{1}{c|}{0.90\%}                    & 30.2                 & 0.4                  & 0.0                  & 6.8                  \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{2.60\%}                    & 45.4                 & 24.0                 & 20.0                 & \multicolumn{1}{c|}{43.9}                & \multicolumn{1}{c|}{1.80\%}                    & 30.2                 & 0.4                  & 0.0                  & 6.8                  \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{5.20\%}                    & 42.5                 & 23.6                 & 20.8                 & \multicolumn{1}{c|}{38.2}                & \multicolumn{1}{c|}{3.60\%}                    & 33.2                 & 17.9                 & 8.8                  & 25.5                 \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{SFGC}}    & \multicolumn{1}{c|}{1.30\%}                    & 46.7                 & 19.9                 & 18.8                 & \multicolumn{1}{c|}{43.4}                & \multicolumn{1}{c|}{0.90\%}                    &                      &                      &                      &                      \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{2.60\%}                    & 56.8                 & 27.4                 & 27.6                 & \multicolumn{1}{c|}{52.8}                & \multicolumn{1}{c|}{1.80\%}                    &                      &                      &                      &                      \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{5.20\%}                    & 47.7                 & 19.0                 & 16.9                 & \multicolumn{1}{c|}{45.3}                & \multicolumn{1}{c|}{3.60\%}                    &                      &                      &                      &                      \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{GEOM}}    & \multicolumn{1}{c|}{1.30\%}                    & 41.4                 & 16.9                 & 16.2                 & \multicolumn{1}{c|}{38.6}                & \multicolumn{1}{c|}{0.90\%}                    &                      &                      &                      &                      \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{2.60\%}                    & 44.1                 & 18.1                 & 18.1                 & \multicolumn{1}{c|}{38.8}                & \multicolumn{1}{c|}{1.80\%}                    &                      &                      &                      &                      \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{5.20\%}                    & 22.8                 & 1.8                  & 1.2                  & \multicolumn{1}{c|}{20.9}                & \multicolumn{1}{c|}{3.60\%}                    &                      &                      &                      &                      \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{GCDM}}    & \multicolumn{1}{c|}{1.30\%}                    & 41.4                 & 16.9                 & 16.2                 & \multicolumn{1}{c|}{38.6}                & \multicolumn{1}{c|}{0.90\%}                    &                      &                      &                      &                      \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{2.60\%}                    & 44.1                 & 18.1                 & 18.1                 & \multicolumn{1}{c|}{38.8}                & \multicolumn{1}{c|}{1.80\%}                    &                      &                      &                      &                      \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{5.20\%}                    & 22.8                 & 1.8                  & 1.2                  & \multicolumn{1}{c|}{20.9}                & \multicolumn{1}{c|}{3.60\%}                    &                      &                      &                      &                      \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{DM}}      & \multicolumn{1}{c|}{1.30\%}                    & 23.5                 & 2.1                  & 1.1                  & \multicolumn{1}{c|}{17.7}                & \multicolumn{1}{c|}{0.90\%}                    &                      &                      &                      &                      \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{2.60\%}                    & 45.3                 & 19.1                 & 17.7                 & \multicolumn{1}{c|}{42.9}                & \multicolumn{1}{c|}{1.80\%}                    &                      &                      &                      &                      \\
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{5.20\%}                    & 25.9                 & 4.5                  & 3.5                  & \multicolumn{1}{c|}{20.0}                & \multicolumn{1}{c|}{3.60\%}                    &                      &                      &                      &                      \\ \midrule
                                              & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                                          & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
                                              & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                                          & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
                                              & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                                          & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
                                              & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &                                          & \multicolumn{1}{l}{}                           & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}
\end{tabular}
\end{table}


==> table/alg.tex <==
% \IncMargin{1em}
% \begin{algorithm}[htbp]
%     \caption{Overall training process of \modelname.}
%     \label{alg:alg}
%     \KwIn{Dynamic graph $\mathbf{DG} = (\{ \mathcal{G} \}_{t=1}^{T})$ with labels $\mathbf{Y}^{1:T}$ of link occurrence; Number of training epochs $E$; Number of intervention times $S$; Hyperparameters $\alpha$ and $\beta$.}
%     \KwOut{Optimized model $f_{\boldsymbol{\theta}}^{\star}$; Predicted label $Y^{T}$ of link occurrence at time $T+1$.}
%     \BlankLine 
%     Initialize parameters randomly\;
%     \For{$i=1,2,\cdots,E$}{
%          \vspace{0.5em}
%         \tcp{Model environment-aware representations and infer distributions} 
%         Obtain representations for each node at each time with the support of $\mathbf{e}$, as $\mathbf{z}_{v}^{\mathbf{e},t} \gets$ Eq. \eqref{eq:repre}\;
%         Establish the observed environment samples library $\mathcal{S}_{\mathrm{ob}} \gets$ Eq. \eqref{eq:sob}\;
%         Infer the distribution $p_\omega(\mathbf{e})$ with $\mathcal{L}_{\mathrm{ECVAE}} \gets$ Eq. \eqref{eq:ecvae} and generate samples library $\mathcal{S}_{\mathrm{ge}}$\; \vspace{0.5em}
%         % \BlankLine 
%         \tcp{Extrapolate spatio-temporal invariant patterns} 
%         Learn the invariance threshold $\delta_v \gets$ Eq. \eqref{eq:delta} by function $\mathbb{I}(\cdot) \gets$ Eq. \eqref{eq:trans}\;
%         Recognize the invariant/variant patterns for each node, as $\mathbf{e}_v^{I}, \mathbf{e}_v^{V} \gets$ Eq. \eqref{eq:evi}\;
%         Calculate task loss depending on the invariant patterns, as $\mathcal{L}_{\mathrm{task}} \gets$ Eq. \eqref{eq:taskloss}\;
%         % \BlankLine 
%          \vspace{0.5em}\tcp{Perform causal inference with intervention}
%         \For{$j=1,2,\cdots,S$}{
%             Sample $|\mathbf{e}_v^V|$ items from $\mathcal{S}_{\mathrm{ob}} \cup \mathcal{S}_{\mathrm{ge}}$ and perform intervention for each node, as Eq. \eqref{eq:intervention}\;
%             Calculate intervention loss, as $\mathcal{L}_{\mathrm{interv}} \gets$ Eq. \eqref{eq:intervloss}\;
%         }
%          \vspace{0.5em}\tcp{Optimize}
%         Calculate the overall loss, as $\mathcal{L} \gets$ Eq. \eqref{eq:final2}\;
%         Update model parameters by minimizing $\mathcal{L}$.
%     }
% \end{algorithm}
% \DecMargin{1em}

\IncMargin{1em}
\begin{algorithm}[h]
    \caption{Overall training process of \modelname.}
    \label{alg:alg}
    \KwIn{Dynamic graph $\mathbf{DG} = (\{ \mathcal{G} \}_{t=1}^{T})$ with labels $\mathbf{Y}^{1:T}$ of link occurrence; Number of training epochs $E$; Number of intervention times $S$; Hyperparameters $\alpha$ and $\beta$.}
    \KwOut{Optimized model $f_{\boldsymbol{\theta}}^{\star}$; Predicted label $Y^{T}$ of link occurrence at time $T+1$.}
    \BlankLine 
    Initialize parameters randomly\;
    \For{$i=1,2,\cdots,E$}{
         \vspace{0.5em}
        \tcp{Environments Modeling and Inferring} 
        Obtain representations for each node at each time with the support of $\mathbf{e}$, as $\mathbf{z}_{v}^{\mathbf{e},t} \gets$ Eq. \eqref{eq:repre}\;
        Establish the observed environment samples library $\mathcal{S}_{\mathrm{ob}} \gets$ Eq. \eqref{eq:sob}\;
        Infer the distribution $p_\omega(\mathbf{e})$ with $\mathcal{L}_{\mathrm{ECVAE}} \gets$ Eq. \eqref{eq:ecvae} and generate samples library $\mathcal{S}_{\mathrm{ge}}$\; \vspace{0.5em}
        % \BlankLine 
        \tcp{Environments Extrapolating} 
        Learn the invariance threshold $\delta_v \gets$ Eq. \eqref{eq:delta} by function $\mathbb{I}(\cdot) \gets$ Eq. \eqref{eq:trans}\;
        Recognize the invariant/variant patterns for each node, as $\mathcal{P}_\mathbf{e}^{I}(v)$, $\mathcal{P}_\mathbf{e}^{V}(v) \gets$ Eq. \eqref{eq:evi}\;
        Calculate task loss depending on the invariant patterns, as $\mathcal{L}_{\mathrm{task}} \gets$ Eq. \eqref{eq:taskloss}\;
        % \BlankLine 
         \vspace{0.5em}\tcp{Environments Generalizing}
        \For{$j=1,2,\cdots,S$}{
            Sample items from $\mathcal{S}_{\mathrm{ob}} \cup \mathcal{S}_{\mathrm{ge}}$ and perform intervention for each node, as Eq. \eqref{eq:intervention}\;
            Calculate intervention loss, as $\mathcal{L}_{\mathrm{risk}} \gets$ Eq. \eqref{eq:intervloss}\;
        }
         \vspace{0.5em}\tcp{Optimize}
        Calculate the overall loss, as $\mathcal{L} \gets$ Eq. \eqref{eq:final2}\;
        Update model parameters by minimizing $\mathcal{L}$.
    }
\end{algorithm}
\DecMargin{1em}

==> table/cross_archi.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Comparison of results using SGC and GCN as condensing architectures and testing the condensed graph under different downstream architectures. The best results are in \textbf{bold}, and the runner-up results are \underline{underlined}.}
\label{tab:trans_arch}
% \small
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccccc|c@{}}
\toprule
Methods                                       & C \textbackslash{} T & SGC              & GCN              & SAGE             & APPNP            & Cheby            & MLP              & GT          & Avg.             \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{GCond}}   & SGC & 72.6             & 62.9             & 60.9             & 72.4             & 72.0             & 44.0             & 25.0             & 58.5             \\
\multicolumn{1}{c|}{}                         & GCN & 75.6             & 64.5             & 63.7             & 73.0             & 74.8             & 60.0             & 20.8             & 61.8             \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{DosCond}} & SGC & 77.4             & 77.4             & 77.6             & 74.1             & 59.1             & \underline{76.8} & 21.1             & 66.2             \\
\multicolumn{1}{c|}{}                         & GCN & 78.3             & \underline{78.3} & 79.0             & 66.4             & 58.1             & \textbf{76.9}    & 20.1             & 65.3             \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{SGDD}}    & SGC & \textbf{79.7}    & 48.5             & 44.4             & 80.1             & 14.5             & 40.0             & \underline{25.7} & 47.6             \\
\multicolumn{1}{c|}{}                         & GCN & \underline{79.3} & 53.9             & 29.0             & 79.4             & 23.2             & 39.2             & \textbf{34.2}    & 48.3             \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{SFGC}}    & SGC & 77.3             & \textbf{79.0}    & \textbf{81.1}    & \textbf{81.0}    & \underline{79.2} & 74.0             & \todo{nan}              & \textbf{78.6}    \\
\multicolumn{1}{c|}{}                         & GCN & 77.9             & 78.1             & \underline{80.1} & \underline{80.9} & \textbf{79.5}    & 72.3             & \todo{nan}              & \underline{78.1} \\ \bottomrule
\end{tabular}%
% }
\end{table}

==> table/datasets.tex <==
\begin{table}[htbp]
\caption{Statistics of the real-world datasets.}
\label{tab:data}
\centering
\resizebox{\linewidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule
    \textbf{Dataset} & \textbf{\# Nodes} & \textbf{\# Links}  & \textbf{\makecell{\# Graph\\Snapshots}} & \textbf{\makecell{Temporal\\Granularity}}  & \textbf{In-distribution Attributes}& \textbf{\makecell{Shifted\\Attribute}} \\
    \midrule
    \renewcommand{\arraystretch}{10}
    COLLAB & 23,035 & 151,790  & 16   & year & \makecell{Database, Medical Informatics,\\Theory, Visualization} & Data Mining\\
    \specialrule{0em}{1.2pt}{1.2pt}
    Yelp  & 13,095 & 65,375  & 24   & month  & \makecell{American (New) Food, Fast Food\\Sushi Bars, Coffee~\&~Tea} & Pizza\\
    \specialrule{0em}{1.2pt}{1.2pt}
    ACT   & 19,008 & 202,339  & 30   & day  & Attributes 1-4 & Attribute 5\\
    \bottomrule
    \end{tabular}%
}
\end{table}


==> table/graph-cls-backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{\textbf{Graph classification performance on GIN} (mean±std) across datasets with varying condensation ratios $r$. 
The best results are shown in \colorbox{gray!45}{\textbf{bold}} and the runner-ups are shown in \colorbox{gray!20}{\underline{underlined}}. 
% To better visualize improvements over the whole dataset results, we use 
\textcolor{red}{Red} color
highlights entries that exceed the whole dataset values. 
% Parameters were adjusted to match Mirage's dataset disk size with that condensed by DosCond.
}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Dataset}}                                                                  & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Graph\\ /Cls\end{tabular}}} & \multirow{2}{*}{\textbf{Ratio($r$)}} & \multicolumn{3}{c}{\textbf{Traditional Core-set methods}}                                                                                                                                                   & \textbf{Gradient}                                                         & \textbf{KRR}                                                                              & \textbf{CTC}                                                                           & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Whole\\ Dataset\end{tabular}}} \\ \cmidrule(lr){4-9}
                                                                                                   &                                                                                &                                      & \textbf{Random}                                               & \textbf{Herding}                                          & \multicolumn{1}{c|}{\textbf{K-Center}}                                          & \multicolumn{1}{c|}{\textbf{DosCond}}                                     & \multicolumn{1}{c|}{\textbf{KiDD}}                                                        & \textbf{Mirage}                                                                        &                                                                                   \\ \midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\nci\\ Acc. (\%)\end{tabular}}}     & 1                                                                              & \multicolumn{1}{c|}{0.06\%}          & 50.90$_{\pm 2.10}$                                            & {\cellcolor{gray!20}\underline{51.90}$_{\pm 1.60}$}       & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{51.90}$_{\pm 1.60}$}}        & \multicolumn{1}{c|}{49.20$_{\pm 1.10}$}                                   & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{61.40}$_{\pm 0.50}$}}}            & \multicolumn{1}{c|}{50.80$_{\pm 2.20}$}                                                & \multirow{5}{*}{80.0$_{\pm 1.8}$}                                                 \\
\multicolumn{1}{c|}{}                                                                              & 5                                                                              & \multicolumn{1}{c|}{0.24\%}          & 52.10$_{\pm 1.00}$                                            & {\cellcolor{gray!20}\underline{60.50}$_{\pm 2.40}$}       & \multicolumn{1}{c|}{47.00$_{\pm 1.10}$}                                         & \multicolumn{1}{c|}{51.10$_{\pm 0.80}$}                                   & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{63.20}$_{\pm 0.20}$}}}            & \multicolumn{1}{c|}{51.30$_{\pm 1.10}$}                                                &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 10                                                                             & \multicolumn{1}{c|}{0.49\%}          & 55.60$_{\pm 1.90}$                                            & {\cellcolor{gray!20}\underline{61.80}$_{\pm 1.50}$}       & \multicolumn{1}{c|}{49.40$_{\pm 1.80}$}                                         & \multicolumn{1}{c|}{50.30$_{\pm 1.30}$}                                   & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{64.20}$_{\pm 0.10}$}}}            & \multicolumn{1}{c|}{51.70$_{\pm 1.40}$}                                                &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 20                                                                             & \multicolumn{1}{c|}{0.97\%}          & 58.70$_{\pm 1.40}$                                            & \textbf{{\cellcolor{gray!45}\textbf{60.90}$_{\pm 1.90}$}} & \multicolumn{1}{c|}{55.20$_{\pm 1.60}$}                                         & \multicolumn{1}{c|}{50.30$_{\pm 1.30}$}                                   & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{60.90}$_{\pm 0.70}$}}}            & \multicolumn{1}{c|}{52.10$_{\pm 2.20}$}                                                &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 50                                                                             & \multicolumn{1}{c|}{2.43\%}          & 61.10$_{\pm 1.20}$                                            & 59.00$_{\pm 1.50}$                                        & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{62.70}$_{\pm 1.50}$}}        & \multicolumn{1}{c|}{50.30$_{\pm 1.30}$}                                   & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{65.40}$_{\pm 0.60}$}}}            & \multicolumn{1}{c|}{52.40$_{\pm 2.70}$}                                                &                                                                                   \\ \midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\dd\\ Acc. (\%)\end{tabular}}}      & 1                                                                              & \multicolumn{1}{c|}{0.21\%}          & 49.70$_{\pm 11.30}$                                           & 58.80$_{\pm 6.10}$                                        & \multicolumn{1}{c|}{58.80$_{\pm 6.10}$}                                         & \multicolumn{1}{c|}{46.30$_{\pm 8.50}$}                                   & \multicolumn{1}{c|}{\textcolor{red}{{\cellcolor{gray!20}\underline{71.30}$_{\pm 1.50}$}}} & \multicolumn{1}{c|}{\textcolor{red}{{\cellcolor{gray!45}\textbf{74.00}$_{\pm 0.40}$}}} & \multirow{5}{*}{70.1$_{\pm 2.2}$}                                                 \\
\multicolumn{1}{c|}{}                                                                              & 5                                                                              & \multicolumn{1}{c|}{1.06\%}          & 40.80$_{\pm 4.30}$                                            & {\cellcolor{gray!20}\underline{58.70}$_{\pm 5.80}$}       & \multicolumn{1}{c|}{51.30$_{\pm 5.30}$}                                         & \multicolumn{1}{c|}{57.50$_{\pm 5.60}$}                                   & \multicolumn{1}{c|}{\textcolor{red}{{\cellcolor{gray!45}\textbf{70.90}$_{\pm 1.10}$}}}    & \multicolumn{1}{c|}{-}                                                                 &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 10                                                                             & \multicolumn{1}{c|}{2.12\%}          & 63.10$_{\pm 5.20}$                                            & {\cellcolor{gray!20}\underline{64.10}$_{\pm 5.80}$}       & \multicolumn{1}{c|}{53.40$_{\pm 3.10}$}                                         & \multicolumn{1}{c|}{46.30$_{\pm 8.50}$}                                   & \multicolumn{1}{c|}{\textcolor{red}{{\cellcolor{gray!45}\textbf{71.50}$_{\pm 0.50}$}}}    & \multicolumn{1}{c|}{-}                                                                 &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 20                                                                             & \multicolumn{1}{c|}{4.25\%}          & 56.40$_{\pm 4.30}$                                            & {\cellcolor{gray!20}\underline{67.00}$_{\pm 2.60}$}       & \multicolumn{1}{c|}{58.50$_{\pm 5.70}$}                                         & \multicolumn{1}{c|}{40.70$_{\pm 0.00}$}                                   & \multicolumn{1}{c|}{\textcolor{red}{{\cellcolor{gray!45}\textbf{71.20}$_{\pm 0.90}$}}}    & \multicolumn{1}{c|}{-}                                                                 &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 50                                                                             & \multicolumn{1}{c|}{10.62\%}         & 58.90$_{\pm 6.30}$                                            & {\cellcolor{gray!20}\underline{68.40}$_{\pm 4.00}$}       & \multicolumn{1}{c|}{62.30$_{\pm 2.50}$}                                         & \multicolumn{1}{c|}{44.00$_{\pm 6.70}$}                                   & \multicolumn{1}{c|}{\textcolor{red}{{\cellcolor{gray!45}\textbf{71.80}$_{\pm 1.00}$}}}    & \multicolumn{1}{c|}{-}                                                                 &                                                                                   \\ \midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\bace\\ ROC-AUC\end{tabular}}} & 1                                                                              & \multicolumn{1}{c|}{0.17\%}          & 0.468$_{\pm 0.045}$                                           & 0.486$_{\pm 0.035}$                                       & \multicolumn{1}{c|}{0.486$_{\pm 0.035}$}                                        & \multicolumn{1}{c|}{0.512$_{\pm 0.092}$}                                  & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{0.706}$_{\pm 0.000}$}}}           & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{0.590}$_{\pm 0.004}$}}              & \multirow{5}{*}{0.763$_{\pm 0.020}$}                                                 \\
\multicolumn{1}{c|}{}                                                                              & 5                                                                              & \multicolumn{1}{c|}{0.83\%}          & \textbf{{\cellcolor{gray!20}\underline{0.555}$_{\pm 0.079}$}} & 0.470$_{\pm 0.042}$                                       & \multicolumn{1}{c|}{0.553$_{\pm 0.024}$}                                        & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{0.555}$_{\pm 0.079}$}} & \multicolumn{1}{c|}{{\cellcolor{gray!45}\textbf{0.562}$_{\pm 0.000}$}}                    & \multicolumn{1}{c|}{0.419$_{\pm 0.010}$}                                               &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 10                                                                             & \multicolumn{1}{c|}{1.65\%}          & 0.536$_{\pm 0.072}$                                  & 0.532$_{\pm 0.031}$                                       & \multicolumn{1}{c|}{{\cellcolor{gray!45}\textbf{0.594}$_{\pm 0.019}$}}          & \multicolumn{1}{c|}{0.536$_{\pm 0.072}$}                                  & \multicolumn{1}{c|}{{\cellcolor{gray!45}\textbf{0.594}$_{\pm 0.000}$}}                    & \multicolumn{1}{c|}{0.419$_{\pm 0.010}$}                                               &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 20                                                                             & \multicolumn{1}{c|}{3.31\%}          & 0.484$_{\pm 0.080}$                                  & 0.509$_{\pm 0.052}$                                       & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{0.512}$_{\pm 0.031}$}}       & \multicolumn{1}{c|}{0.484$_{\pm 0.080}$}                                  & \multicolumn{1}{c|}{{\cellcolor{gray!45}\textbf{0.640}$_{\pm 0.011}$}}                    & \multicolumn{1}{c|}{0.423$_{\pm 0.011}$}                                               &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 50                                                                             & \multicolumn{1}{c|}{8.26\%}          & 0.503$_{\pm 0.084}$                                           & {\cellcolor{gray!20}\underline{0.625}$_{\pm 0.026}$}      & \multicolumn{1}{c|}{0.595$_{\pm 0.026}$}                                        & \multicolumn{1}{c|}{0.503$_{\pm 0.084}$}                                  & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{0.723}$_{\pm 0.011}$}}}           & \multicolumn{1}{c|}{-}                                                                 &                                                                                   \\ \midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\bbbp\\ ROC-AUC\end{tabular}}} & 1                                                                              & \multicolumn{1}{c|}{0.12\%}          & 0.510$_{\pm 0.013}$                                           & 0.532$_{\pm 0.015}$                                       & \multicolumn{1}{c|}{0.532$_{\pm 0.015}$}                                        & \multicolumn{1}{c|}{0.546$_{\pm 0.026}$}                                  & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{0.616}$_{\pm 0.000}$}}}           & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{0.592}$_{\pm 0.004}$}}              & \multirow{5}{*}{0.635$_{\pm 0.017}$}                                                 \\
\multicolumn{1}{c|}{}                                                                              & 5                                                                              & \multicolumn{1}{c|}{0.61\%}          & 0.522$_{\pm 0.014}$                                           & 0.546$_{\pm 0.020}$                                       & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{0.581}$_{\pm 0.022}$}}       & \multicolumn{1}{c|}{0.519$_{\pm 0.041}$}                                  & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{0.607}$_{\pm 0.005}$}}}           & \multicolumn{1}{c|}{0.431$_{\pm 0.013}$}                                               &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 10                                                                             & \multicolumn{1}{c|}{1.23\%}          & 0.508$_{\pm 0.018}$                                           & 0.578$_{\pm 0.017}$                                       & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{0.619}$_{\pm 0.027}$}}       & \multicolumn{1}{c|}{0.505$_{\pm 0.028}$}                                  & \multicolumn{1}{c|}{{\cellcolor{gray!45}\textbf{0.663}$_{\pm 0.000}$}}                    & \multicolumn{1}{c|}{0.465$_{\pm 0.036}$}                                               &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 20                                                                             & \multicolumn{1}{c|}{2.45\%}          & 0.567$_{\pm 0.010}$                                           & 0.533$_{\pm 0.009}$                                       & \multicolumn{1}{c|}{0.546$_{\pm 0.012}$}                                        & \multicolumn{1}{c|}{0.493$_{\pm 0.031}$}                                  & \multicolumn{1}{c|}{{\cellcolor{gray!45}\textbf{0.677}$_{\pm 0.001}$}}                    & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{0.610}$_{\pm 0.022}$}}              &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 50                                                                             & \multicolumn{1}{c|}{6.13\%}          & {\cellcolor{gray!20}\underline{0.595}$_{\pm 0.014}$}          & 0.552$_{\pm 0.018}$                                       & \multicolumn{1}{c|}{0.594$_{\pm 0.016}$}                                        & \multicolumn{1}{c|}{0.509$_{\pm 0.015}$}                                  & \multicolumn{1}{c|}{{\cellcolor{gray!45}\textbf{0.684}$_{\pm 0.009}$}}                    & \multicolumn{1}{c|}{0.590$_{\pm 0.031}$}                                               &                                                                                   \\ \midrule
\multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\hiv\\ ROC-AUC\end{tabular}}}  & 1                                                                              & \multicolumn{1}{c|}{0.01\%}          & 0.366$_{\pm 0.087}$                                           & 0.462$_{\pm 0.072}$                                       & \multicolumn{1}{c|}{0.462$_{\pm 0.072}$}                                        & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{0.674}$_{\pm 0.131}$}} & \multicolumn{1}{c|}{0.664$_{\pm 0.016}$}                                                  & \multicolumn{1}{c|}{{\cellcolor{gray!45}\textbf{0.710}$_{\pm 0.009}$}}                 & \multirow{5}{*}{0.701$_{\pm 0.028}$}                                                 \\
\multicolumn{1}{c|}{}                                                                              & 5                                                                              & \multicolumn{1}{c|}{0.03\%}          & 0.501$_{\pm 0.051}$                                           & 0.496$_{\pm 0.044}$                                       & \multicolumn{1}{c|}{0.519$_{\pm 0.096}$}                                        & \multicolumn{1}{c|}{0.369$_{\pm 0.175}$}                                  & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{0.657}$_{\pm 0.005}$}}                 & \multicolumn{1}{c|}{{\cellcolor{gray!45}\textbf{0.703}$_{\pm 0.012}$}}                 &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 10                                                                             & \multicolumn{1}{c|}{0.06\%}          & {\cellcolor{gray!20}\underline{0.554}$_{\pm 0.031}$}          & 0.458$_{\pm 0.058}$                                       & \multicolumn{1}{c|}{0.471$_{\pm 0.054}$}                                        & \multicolumn{1}{c|}{0.457$_{\pm 0.214}$}                                  & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{0.632}$_{\pm 0.000}$}}}           & \multicolumn{1}{c|}{0.513$_{\pm 0.055}$}                                               &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 20                                                                             & \multicolumn{1}{c|}{0.12\%}          & 0.621$_{\pm 0.022}$                                           & 0.582$_{\pm 0.027}$                                       & \multicolumn{1}{c|}{0.627$_{\pm 0.050}$}                                        & \multicolumn{1}{c|}{0.281$_{\pm 0.007}$}                                  & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{0.648}$_{\pm 0.025}$}}}           & \multicolumn{1}{c|}{{\cellcolor{gray!20}\underline{0.633}$_{\pm 0.048}$}}              &                                                                                   \\
\multicolumn{1}{c|}{}                                                                              & 50                                                                             & \multicolumn{1}{c|}{0.30\%}          & {\cellcolor{gray!20}\underline{0.625}$_{\pm 0.062}$}          & 0.600$_{\pm 0.034}$                                       & \multicolumn{1}{c|}{\textbf{{\cellcolor{gray!45}\textbf{0.680}$_{\pm 0.049}$}}} & \multicolumn{1}{c|}{0.455$_{\pm 0.214}$}                                  & \multicolumn{1}{c|}{0.587$_{\pm 0.038}$}                                                  & \multicolumn{1}{c|}{0.588$_{\pm 0.067}$}                                               &                                                                                   \\ \midrule
\multicolumn{10}{l}{\makecell[l]{$*$\textit{Mirage} cannot directly generate graphs with the required ratio. Thus, we search the parameter space and aligned the\\~~generated graph to match \textit{DosCond}'s disk usage as substitution (see Appendix~\ref{app:rq1}).}}                                          
\end{tabular}%
}
\end{table}

==> table/graph_main.tex <==
\begin{table}[htbp]
\caption{Graph Classification on GIN Performance comparison (mean±std) across datasets with varying condensation ratios.}
\label{tab:GIN_GC_ratios}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}ccccccccc@{}}
\toprule
Dataset                                                                            & Graphs/Cls & Ratio                      & Random               & Herding        & K-Center             & DosCond           & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}KiDD} & WholeDataset                                       \\ \midrule
                                                                                   & 1          & 0.06\%                     & 50.9±2.1             & {\ul 51.9±1.6} & {\ul 51.9±1.6}       & 49.2±1.1          & \multicolumn{1}{c|}{\textbf{61.4±0.5}}            &                                                    \\
                                                                                   & 5          & 0.24\%                     & 52.1±1.0             & {\ul 60.5±2.4} & 47.0±1.1             & 51.1±0.8          & \multicolumn{1}{c|}{\textbf{63.2±0.2}}            &                                                    \\
                                                                                   & 10         & 0.49\%                     & 55.6±1.9             & {\ul 61.8±1.5} & 49.4±1.8             & 50.3±1.3          & \multicolumn{1}{c|}{\textbf{64.2±0.1}}            &                                                    \\
                                                                                   & 20         & 0.97\%                     & 58.7±1.4             & {\ul 60.9±1.9} & 55.2±1.6             & 50.3±1.3          & \multicolumn{1}{c|}{\textbf{60.9±0.7}}      &                                                    \\
\multirow{-5}{*}{NCI1(ACC)}                                                        & 50         & 2.43\%                     & 61.1±1.2             & 59.0±1.5       & {\ul 62.7±1.5}       & 50.3±1.3          & \multicolumn{1}{c|}{\textbf{65.4±0.6}}            & \multirow{-5}{*}{80.0±1.8}                         \\ \midrule
                                                                                   & 1          & 0.21\%                     & 49.7±11.3            & {\ul 58.8±6.1} & {\ul 58.8±6.1}       & 46.3±8.5          & \multicolumn{1}{c|}{\textbf{71.3±1.5}}            & \cellcolor[HTML]{FFFFFF}                           \\
                                                                                   & 5          & 1.06\%                     & {\ul 61.8±5.6}       & 58.7±5.8       & 51.3±5.3             & 57.5±5.6          & \multicolumn{1}{c|}{\textbf{70.9±1.1}}            & \cellcolor[HTML]{FFFFFF}                           \\
                                                                                   & 10         & 2.12\%                     & 63.1±5.2             & {\ul 64.1±5.8} & 53.4±3.1             & 46.3±8.5          & \multicolumn{1}{c|}{\textbf{71.5±0.5}}            & \cellcolor[HTML]{FFFFFF}                           \\
                                                                                   & 20         & 4.25\%                     & 56.4±4.3             & {\ul 67.0±2.6} & 58.5±5.7             & 40.7±0.0          & \multicolumn{1}{c|}{\textbf{71.2±0.9}}            & \cellcolor[HTML]{FFFFFF}                           \\
\multirow{-5}{*}{DD(ACC)}                                                          & 50         & 10.62\%                    & 58.9±6.3             & {\ul 68.4±4.0} & 62.3±2.5             & 44.0±6.7          & \multicolumn{1}{c|}{\textbf{71.8±1.0}}            & \multirow{-5}{*}{\cellcolor[HTML]{FFFFFF}76.9±2.2} \\ \midrule
                                                                                   & 1          & \multicolumn{1}{l}{0.17\%} & 0.468±0.045          & 0.486±0.035    & 0.486±0.035          & {\ul 0.512±0.092} & \multicolumn{1}{c|}{\textbf{0.706±0.000}}         &                                                    \\
                                                                                   & 5          & \multicolumn{1}{l}{0.83\%} & \textbf{0.605±0.019} & 0.470±0.042    & 0.553±0.024          & 0.555±0.079       & \multicolumn{1}{c|}{{\ul 0.562±0.000}}            &                                                    \\
                                                                                   & 10         & \multicolumn{1}{l}{1.65\%} & \textbf{0.618±0.017} & 0.532±0.031    & 0.594±0.019          & 0.536±0.072       & \multicolumn{1}{c|}{{\ul 0.594±0.000}}            &                                                    \\
                                                                                   & 20         & \multicolumn{1}{l}{3.31\%} & \textbf{0.714±0.012} & 0.509±0.052    & 0.512±0.031          & 0.484±0.080       & \multicolumn{1}{c|}{{\ul 0.640±0.011}}            &                                                    \\
\multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}ogbg-molbace\\ (ROC-AUC)\end{tabular}} & 50         & \multicolumn{1}{l}{8.26\%} & {\ul 0.693±0.016}    & 0.625±0.026    & 0.595±0.026          & 0.503±0.084       & \multicolumn{1}{c|}{\textbf{0.723±0.011}}         & \multirow{-5}{*}{0.763±0.020}                      \\ \midrule
                                                                                   & 1          & \multicolumn{1}{l}{0.12\%} & 0.510±0.013          & 0.532±0.015    & 0.532±0.015          & {\ul 0.546±0.026} & \multicolumn{1}{c|}{\textbf{0.616±0.000}}         &                                                    \\
                                                                                   & 5          & \multicolumn{1}{l}{0.61\%} & 0.522±0.014          & 0.546±0.020    & {\ul 0.581±0.022}    & 0.519±0.041       & \multicolumn{1}{c|}{\textbf{0.607±0.005}}         &                                                    \\
                                                                                   & 10         & \multicolumn{1}{l}{1.23\%} & 0.508±0.018          & 0.578±0.017    & {\ul 0.619±0.027}    & 0.505±0.028       & \multicolumn{1}{c|}{\textbf{0.663±0.000}}         &                                                    \\
                                                                                   & 20         & \multicolumn{1}{l}{2.45\%} & {\ul 0.567±0.010}    & 0.533±0.009    & 0.546±0.012          & 0.493±0.031       & \multicolumn{1}{c|}{\textbf{0.677±0.001}}         &                                                    \\
\multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}ogbg-molbbbp\\ (ROC-AUC)\end{tabular}} & 50         & \multicolumn{1}{l}{6.13\%} & {\ul 0.595±0.014}    & 0.552±0.018    & 0.594±0.016          & 0.509±0.015       & \multicolumn{1}{c|}{\textbf{0.684±0.009}}         & \multirow{-5}{*}{0.635±0.017}                      \\ \midrule
                                                                                   & 1          & \multicolumn{1}{l}{0.01\%} & \textbf{0.721±0.023} & 0.462±0.072    & 0.462±0.072          & {\ul 0.674±0.131} & \multicolumn{1}{c|}{0.664±0.016}                  &                                                    \\
                                                                                   & 5          & \multicolumn{1}{l}{0.03\%} & 0.501±0.051          & 0.496±0.044    & {\ul 0.519±0.096}    & 0.369±0.175       & \multicolumn{1}{c|}{\textbf{0.657±0.005}}         &                                                    \\
                                                                                   & 10         & \multicolumn{1}{l}{0.06\%} & {\ul 0.554±0.031}    & 0.458±0.058    & 0.471±0.054          & 0.457±0.214       & \multicolumn{1}{c|}{\textbf{0.632±0.000}}         &                                                    \\
                                                                                   & 20         & \multicolumn{1}{l}{0.12\%} & 0.621±0.022          & 0.582±0.027    & {\ul 0.627±0.050}    & 0.281±0.007       & \multicolumn{1}{c|}{\textbf{0.648±0.025}}         &                                                    \\
\multirow{-5}{*}{\begin{tabular}[c]{@{}c@{}}ogbg-molhiv\\ (ROC-AUC)\end{tabular}}  & 50         & \multicolumn{1}{l}{0.30\%} & {\ul 0.625±0.062}    & 0.600±0.034    & \textbf{0.680±0.049} & 0.455±0.214       & \multicolumn{1}{c|}{0.587±0.038}                  & \multirow{-5}{*}{0.701±0.028}                      \\ \midrule
                                                                                   &            &                            &                      &                &                      &                   &                                                   &                                                    \\
                                                                                   &            &                            &                      &                &                      &                   &                                                   &                                                    \\
                                                                                   &            &                            &                      &                &                      &                   &                                                   &                                                    \\
                                                                                   &            &                            &                      &                &                      &                   &                                                   &                                                    \\
                                                                                   &            &                            &                      &                &                      &                   &                                                   &                                                    \\
                                                                                   &            &                            &                      &                &                      &                   &                                                   &                                                   
\end{tabular}
}
\end{table}


==> table/main_results_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cc|c|ccc|cc|ccc|cc|c@{}}
\toprule
\multicolumn{2}{c|}{}                                                                                                                                   &                            & \multicolumn{3}{c|}{Traditional Coreset Methods}                                                                                          & \multicolumn{2}{c|}{Distribution}                                                                                                                 & \multicolumn{3}{c|}{Gradient}                                                                                                                                                                                                     & \multicolumn{2}{c|}{Trajectory}                                                                                                                &                                                                           \\ \cmidrule(lr){4-13}
\multicolumn{2}{c|}{}                                                                                                                                   &                            &                                                     &                                                        &                            &                                                                         &                                                                         &                                                                         &                                                        &                                                                                                &                                                                         &                                                                      &                                                                           \\
\multicolumn{2}{c|}{\multirow{-3}{*}{Dataset}}                                                                                                          & \multirow{-3}{*}{Ratio(r)} & \multirow{-2}{*}{Random}                            & \multirow{-2}{*}{Herding}                              & \multirow{-2}{*}{K-Center} & \multirow{-2}{*}{GCDM}                                                  & \multirow{-2}{*}{DM}                                                    & \multirow{-2}{*}{DosCond}                                               & \multirow{-2}{*}{GCond}                                & \multirow{-2}{*}{SGDD}                                                                         & \multirow{-2}{*}{SFGC}                                                  & \multirow{-2}{*}{GEOM}                                               & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Whole\\ Dataset\end{tabular}} \\ \midrule
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.26\%                      & 31.6$_{\pm 1.2}$                                    & 48.6$_{\pm 1.4}$                                       & 48.6$_{\pm 1.4}$           & 39.0$_{\pm 0.4}$                                                        & 35.6$_{\pm 3.9}$                                                        & 78.7$_{\pm 1.3}$                                                        & {\cellcolor{gray!45}\textbf{79.8}$_{\pm 0.7}$}    & 78.6$_{\pm 2.7}$                                                                               & {\cellcolor{gray!20}\underline{78.8}$_{\pm 1.2}$}                  & 50.1$_{\pm 1.2}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.52\%                      & 47.1$_{\pm 1.7}$                                    & 56.0$_{\pm 0.6}$                                       & 44.7$_{\pm 2.7}$           & 42.3$_{\pm 0.7}$                                                        & 38.5$_{\pm 4.4}$                                                        & \textcolor{red}{{\cellcolor{gray!20}\underline{81.1}$_{\pm 0.1}$}} & 80.2$_{\pm 0.7}$                                       & \textcolor{red}{{\cellcolor{gray!45}\textbf{81.2}$_{\pm 0.5}$}}                           & 79.2$_{\pm 1.8}$                                                        & 70.5$_{\pm 0.9}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 1.30\%                      & 62.3$_{\pm 1.0}$                                    & 69.9$_{\pm 0.8}$                                       & 62.0$_{\pm 1.3}$           & 63.4$_{\pm 0.1}$                                                        & 63.2$_{\pm 0.5}$                                                        & \textcolor{red}{{\cellcolor{gray!20}\underline{81.2}$_{\pm 0.4}$}} & 80.2$_{\pm 2.2}$                                       & \textcolor{red}{{\cellcolor{gray!45}\textbf{81.6}$_{\pm 0.5}$}}                           & 79.4$_{\pm 0.7}$                                                        & 78.5$_{\pm 1.9}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 2.60\%                      & 72.4$_{\pm 0.5}$                                    & 74.2$_{\pm 0.6}$                                       & 73.5$_{\pm 0.7}$           & 73.4$_{\pm 0.2}$                                                        & 72.6$_{\pm 0.7}$                                                        & 79.6$_{\pm 0.2}$                                                        & 80.5$_{\pm 0.3}$                                       & \textcolor{red}{{\cellcolor{gray!45}\textbf{81.8}$_{\pm 0.2}$}}                           & \textcolor{red}{{\cellcolor{gray!20}\underline{81.7}$_{\pm 0.0}$}} & 76.1$_{\pm 4.7}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 3.90\%                      & 74.6$_{\pm 0.6}$                                    & 76.0$_{\pm 0.6}$                                       & 77.4$_{\pm 0.3}$           & 76.4$_{\pm 0.5}$                                                        & 75.3$_{\pm 0.1}$                                                        & 78.9$_{\pm 0.1}$                                                        & 79.8$_{\pm 0.4}$                                       & \textcolor{red}{{\cellcolor{gray!45}\textbf{82.1}$_{\pm 0.8}$}}                           & \textcolor{red}{{\cellcolor{gray!20}\underline{81.5}$_{\pm 0.5}$}} & 78.3$_{\pm 2.0}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Cora\\ (H=0.81)\end{tabular}}       & 5.20\%                      & 77.1$_{\pm 0.6}$                                    & 76.7$_{\pm 0.4}$                                       & 76.5$_{\pm 0.6}$           & 78.4$_{\pm 0.0}$                                                        & 77.9$_{\pm 0.2}$                                                        & 79.7$_{\pm 0.6}$                                                        & 77.8$_{\pm 3.6}$                                       & \textcolor{red}{{\cellcolor{gray!45}\textbf{82.0}$_{\pm 1.4}$}}                           & \textcolor{red}{{\cellcolor{gray!20}\underline{81.4}$_{\pm 0.0}$}} & 80.4$_{\pm 0.8}$                                                     & \multirow{-6}{*}{80.8±0.3}                                                \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.05\%                      & 45.2$_{\pm 1.7}$                                    & 54.6$_{\pm 2.4}$                                       & 50.7$_{\pm 2.2}$           & 61.1$_{\pm 0.4}$                                                        & 60.6$_{\pm 0.7}$                                                        & 50.1$_{\pm 1.8}$                                                        & {\cellcolor{gray!20}\underline{84.4}$_{\pm 2.6}$} & 83.6$_{\pm 1.7}$                                                                               & {\cellcolor{gray!45}\textbf{87.2}$_{\pm 2.1}$}                     & 73.6$_{\pm 1.2}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.10\%                      & 53.3$_{\pm 1.6}$                                    & 62.3$_{\pm 1.6}$                                       & 50.1$_{\pm 1.3}$           & 72.3$_{\pm 0.5}$                                                        & 68.7$_{\pm 1.2}$                                                        & 59.5$_{\pm 2.8}$                                                        & {\cellcolor{gray!45}\textbf{84.7}$_{\pm 1.9}$}    & {\cellcolor{gray!20}\underline{83.8}$_{\pm 2.2}$}                                         & 81.5$_{\pm 4.2}$                                                        & 76.2$_{\pm 3.9}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.20\%                      & 65.1$_{\pm 1.2}$                                    & 69.4$_{\pm 2.1}$                                       & 54.2$_{\pm 1.9}$           & 80.8$_{\pm 0.6}$                                                        & 76.7$_{\pm 0.1}$                                                        & 65.8$_{\pm 0.4}$                                                        & 86.3$_{\pm 2.4}$                                       & 88.3$_{\pm 0.5}$                                                                               & {\cellcolor{gray!45}\textbf{90.4}$_{\pm 0.9}$}                     & {\cellcolor{gray!20}\underline{89.9}$_{\pm 0.6}$}               &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.50\%                      & 76.1$_{\pm 1.8}$                                    & 81.4$_{\pm 0.7}$                                       & 67.8$_{\pm 1.3}$           & 86.4$_{\pm 0.1}$                                                        & 84.2$_{\pm 0.2}$                                                        & 65.8$_{\pm 0.4}$                                                        & 87.9$_{\pm 2.7}$                                       & 91.0$_{\pm 0.1}$                                                                               & {\cellcolor{gray!45}\textbf{91.7}$_{\pm 0.2}$}                     & {\cellcolor{gray!45}\textbf{91.7}$_{\pm 0.3}$}                  &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 1.00\%                      & 84.9$_{\pm 0.5}$                                    & 85.9$_{\pm 0.3}$                                       & 74.6$_{\pm 0.8}$           & OOM                                                                     & 78.9$_{\pm 0.7}$                                                        & 78.3$_{\pm 1.3}$                                                        & {\cellcolor{gray!20}\underline{87.2}$_{\pm 1.2}$} & 85.9$_{\pm 0.9}$                                                                               & {\cellcolor{gray!45}\textbf{91.8}$_{\pm 0.2}$}                     & OOM                                                                  &                                                                           \\
\multicolumn{1}{c|}{}                                                 & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Reddit\\ (H=0.78)\end{tabular}}     & 5.00\%                      & {\cellcolor{gray!45}\textbf{92.3}$_{\pm 0.1}$} & {\cellcolor{gray!20}\underline{91.9}$_{\pm 0.1}$} & 88.4$_{\pm 0.3}$           & OOM                                                                     & OOM                                                                     & OOM                                                                     & OOM                                                    & OOM                                                                                            & {\cellcolor{gray!20}\underline{91.9}$_{\pm 0.7}$}                  & OOM                                                                  & \multirow{-6}{*}{94.0±0.2}                                                \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.18\%                      & 39.3$_{\pm 1.9}$                                    & 36.6$_{\pm 2.6}$                                       & 36.6$_{\pm 2.6}$           & 30.6$_{\pm 2.5}$                                                        & 32.1$_{\pm 1.5}$                                                        & \textcolor{red}{{\cellcolor{gray!45}\textbf{71.8}$_{\pm 0.1}$}}    & 71.3$_{\pm 0.6}$                                       & {\color[HTML]{0D0D0D} {\cellcolor{gray!20}\underline{71.7}$_{\pm 3.2}$}}                  & 70.7$_{\pm 1.1}$                                                        & 63.7$_{\pm 0.4}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.36\%                      & 44.1$_{\pm 2.0}$                                    & 41.5$_{\pm 2.6}$                                       & 38.7$_{\pm 3.2}$           & 36.2$_{\pm 2.0}$                                                        & 43.3$_{\pm 1.3}$                                                        & \textcolor{red}{{\cellcolor{gray!20}\underline{73.1}$_{\pm 0.3}$}} & 70.4$_{\pm 1.8}$                                       & {\color[HTML]{0D0D0D} \textcolor{red}{{\cellcolor{gray!45}\textbf{73.3}$_{\pm 3.3}$}}}    & 70.9$_{\pm 1.6}$                                                        & 69.8$_{\pm 0.1}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.90\%                      & 49.3$_{\pm 1.0}$                                    & 56.5$_{\pm 1.3}$                                       & 51.4$_{\pm 1.4}$           & 52.6$_{\pm 1.1}$                                                        & 53.7$_{\pm 0.3}$                                                        & \textcolor{red}{{\cellcolor{gray!45}\textbf{73.0}$_{\pm 0.4}$}}    & 70.7$_{\pm 0.9}$                                       & {\color[HTML]{0D0D0D} \textcolor{red}{{\cellcolor{gray!20}\underline{72.8}$_{\pm 0.6}$}}} & 70.7$_{\pm 0.5}$                                                        & 70.5$_{\pm 0.3}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 1.80\%                      & 57.4$_{\pm 0.7}$                                    & 68.4$_{\pm 0.8}$                                       & 61.4$_{\pm 1.2}$           & 64.7$_{\pm 0.6}$                                                        & 66.4$_{\pm 0.2}$                                                        & {\cellcolor{gray!20}\underline{71.6}$_{\pm 0.6}$}                  & 70.2$_{\pm 1.4}$                                       & {\color[HTML]{0D0D0D} \textcolor{red}{{\cellcolor{gray!45}\textbf{73.6}$_{\pm 0.6}$}}}    & 70.4$_{\pm 1.2}$                                                        & 67.5$_{\pm 0.6}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 2.70\%                      & 66.2$_{\pm 1.0}$                                    & 68.1$_{\pm 0.8}$                                       & 67.5$_{\pm 0.8}$           & 69.2$_{\pm 1.6}$                                                        & 68.5$_{\pm 0.0}$                                                        & {\cellcolor{gray!20}\underline{71.7}$_{\pm 1.0}$}                  & 67.7$_{\pm 0.2}$                                       & {\color[HTML]{0D0D0D} \textcolor{red}{{\cellcolor{gray!45}\textbf{72.1}$_{\pm 0.5}$}}}    & 71.0$_{\pm 1.0}$                                                        & 70.9$_{\pm 0.5}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Citeseer\\ (H=0.74)\end{tabular}}   & 3.60\%                      & 69.2$_{\pm 0.3}$                                    & 69.1$_{\pm 0.7}$                                       & 69.3$_{\pm 0.7}$           & 69.3$_{\pm 0.4}$                                                        & 70.4$_{\pm 0.4}$                                                        & \textcolor{red}{{\cellcolor{gray!20}\underline{72.4}$_{\pm 0.3}$}} & 68.4$_{\pm 1.6}$                                       & {\color[HTML]{0D0D0D} \textcolor{red}{{\cellcolor{gray!45}\textbf{73.3}$_{\pm 1.2}$}}}    & 70.6$_{\pm 0.1}$                                                        & 70.7$_{\pm 0.1}$                                                     & \multirow{-6}{*}{71.7±0.0}                                                \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.05\%                      & 10.7$_{\pm 0.9}$                                    & 32.7$_{\pm 0.9}$                                       & 36.9$_{\pm 1.2}$           & 51.1$_{\pm 0.2}$                                                        & 48.7$_{\pm 0.0}$                                                        & 59.5$_{\pm 1.0}$                                                        & 60.0$_{\pm 0.0}$                                       & 59.7$_{\pm 0.2}$                                                                               & {\cellcolor{gray!45}\textbf{68.2}$_{\pm 2.3}$}                     & {\cellcolor{gray!20}\underline{64.5}$_{\pm 0.9}$}               &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.10\%                      & 36.5$_{\pm 1.1}$                                    & 41.6$_{\pm 1.0}$                                       & 40.3$_{\pm 0.9}$           & 55.9$_{\pm 1.5}$                                                        & 55.0$_{\pm 0.0}$                                                        & 60.9$_{\pm 0.8}$                                                        & 59.5$_{\pm 1.1}$                                       & 56.1$_{\pm 3.4}$                                                                               & {\cellcolor{gray!45}\textbf{69.1}$_{\pm 0.7}$}                     & {\cellcolor{gray!20}\underline{64.6}$_{\pm 1.4}$}               &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.20\%                      & 43.2$_{\pm 0.8}$                                    & 48.9$_{\pm 0.8}$                                       & 42.7$_{\pm 1.0}$           & 59.3$_{\pm 0.8}$                                                        & 57.6$_{\pm 0.0}$                                                        & 62.2$_{\pm 0.4}$                                                        & 61.4$_{\pm 0.7}$                                       & 60.9$_{\pm 0.9}$                                                                               & {\cellcolor{gray!45}\textbf{69.0}$_{\pm 0.4}$}                     & {\cellcolor{gray!20}\underline{64.3}$_{\pm 0.0}$}               &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.50\%                      & 48.3$_{\pm 0.4}$                                    & 51.4$_{\pm 0.4}$                                       & 48.3$_{\pm 0.5}$           & 61.0$_{\pm 0.1}$                                                        & 59.9$_{\pm 0.0}$                                                        & 62.1$_{\pm 0.3}$                                                        & 63.0$_{\pm 0.9}$                                       & 63.2$_{\pm 0.2}$                                                                               & {\cellcolor{gray!20}\underline{67.1}$_{\pm 0.0}$}                  & {\cellcolor{gray!45}\textbf{67.2}$_{\pm 0.0}$}                  &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 1.00\%                      & 51.2$_{\pm 0.4}$                                    & 52.0$_{\pm 0.4}$                                       & 50.3$_{\pm 0.5}$           & 61.0$_{\pm 0.0}$                                                        & 60.0$_{\pm 0.0}$                                                        & 61.8$_{\pm 1.3}$                                                        & 62.8$_{\pm 0.0}$                                       & 62.0$_{\pm 2.8}$                                                                               & {\cellcolor{gray!20}\underline{68.4}$_{\pm 1.3}$}                  & {\cellcolor{gray!45}\textbf{69.1}$_{\pm 0.3}$}                  &                                                                           \\
\multicolumn{1}{c|}{}                                                 & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Ogbn-arxiv\\ (H=0.65)\end{tabular}} & 5.00\%                      & 57.2$_{\pm 0.2}$                                    & 56.1$_{\pm 0.2}$                                       & 56.5$_{\pm 0.4}$           & OOM                                                                     & OOM                                                                     & OOM                                                                     & OOM                                                    & OOM                                                                                            & {\cellcolor{gray!20}\underline{69.7}$_{\pm 0.1}$}                  & {\cellcolor{gray!45}\textbf{70.6}$_{\pm 0.5}$}                  & \multirow{-6}{*}{71.5±0.0}                                                \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.05\%                      & 40.5$_{\pm 0.4}$                                    & 41.8$_{\pm 0.6}$                                       & 43.9$_{\pm 0.7}$           & {\cellcolor{gray!20}\underline{45.8}$_{\pm 0.4}$}                  & 44.7$_{\pm 0.5}$                                                        & 40.7$_{\pm 1.1}$                                                        & 44.2$_{\pm 2.3}$                                       & {\cellcolor{gray!45}\textbf{46.6}$_{\pm 0.1}$}                                            & 44.3$_{\pm 0.4}$                                                        & 44.8$_{\pm 0.8}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.10\%                      & 42.0$_{\pm 0.6}$                                    & 41.4$_{\pm 0.6}$                                       & 41.4$_{\pm 0.8}$           & \textcolor{red}{{\cellcolor{gray!45}\textbf{47.5}$_{\pm 0.2}$}}    & 45.4$_{\pm 0.1}$                                                        & 43.2$_{\pm 0.0}$                                                        & 44.2$_{\pm 1.4}$                                       & {\cellcolor{gray!20}\underline{46.8}$_{\pm 0.2}$}                                         & 44.0$_{\pm 1.5}$                                                        & 45.5$_{\pm 0.7}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.20\%                      & 43.1$_{\pm 0.2}$                                    & 41.5$_{\pm 0.7}$                                       & 41.4$_{\pm 0.8}$           & \textcolor{red}{{\cellcolor{gray!45}\textbf{48.8}$_{\pm 0.1}$}}    & 42.8$_{\pm 0.6}$                                                        & 43.9$_{\pm 0.6}$                                                        & 44.4$_{\pm 1.4}$                                       & {\cellcolor{gray!20}\underline{46.8}$_{\pm 0.3}$}                                         & 41.4$_{\pm 5.6}$                                                        & 46.1$_{\pm 0.6}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 0.50\%                      & 43.1$_{\pm 0.3}$                                    & 44.4$_{\pm 0.3}$                                       & 42.6$_{\pm 0.7}$           & \textcolor{red}{{\cellcolor{gray!45}\textbf{49.1}$_{\pm 0.3}$}}    & \textcolor{red}{{\cellcolor{gray!20}\underline{48.6}$_{\pm 0.3}$}} & 45.0$_{\pm 0.3}$                                                        & 44.7$_{\pm 0.6}$                                       & 45.5$_{\pm 0.9}$                                                                               & 46.5$_{\pm 0.1}$                                                        & \textcolor{red}{47.1$_{\pm 0.1}$}                                    &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & 1.00\%                      & 43.0$_{\pm 0.4}$                                    & 44.5$_{\pm 0.6}$                                       & 43.2$_{\pm 0.2}$           & \textcolor{red}{{\cellcolor{gray!20}\underline{49.3}$_{\pm 0.1}$}} & \textcolor{red}{{\cellcolor{gray!45}\textbf{49.6}$_{\pm 0.5}$}}    & 46.0$_{\pm 0.3}$                                                        & 45.1$_{\pm 0.5}$                                       & \textcolor{red}{47.2$_{\pm 0.2}$}                                                              & 46.6$_{\pm 0.0}$                                                        & \textcolor{red}{47.0$_{\pm 0.4}$}                                    &                                                                           \\
\multicolumn{1}{c|}{\multirow{-30}{*}{\rotatebox{90}{Homogeneous}}}   & \multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}Flickr\\ (H=0.24)\end{tabular}}     & 5.00\%                      & 45.2$_{\pm 0.3}$                                    & 44.7$_{\pm 0.4}$                                       & 45.5$_{\pm 0.2}$           & OOM                                                                     & OOM                                                                     & OOM                                                                     & OOM                                                    & OOM                                                                                            & {\cellcolor{gray!20}\underline{45.7}$_{\pm 0.6}$}                  & \textcolor{red}{{\cellcolor{gray!45}\textbf{47.1}$_{\pm 0.3}$}} & \multirow{-6}{*}{46.8±0.2}                                                \\ \midrule
\multicolumn{1}{c|}{}                                                 &                                                                                 & .003\%                      & 83.9$_{\pm 1.7}$                                    & 82.5$_{\pm 1.6}$                                       & 76.3$_{\pm 2.4}$           & 84.8$_{\pm 0.3}$                                                        & 84.8$_{\pm 0.3}$                                                        & 89.3$_{\pm 0.6}$                                                        & 80.6$_{\pm 0.8}$                                       & {\cellcolor{gray!20}\underline{90.3}$_{\pm 2.3}$}                                         & \textcolor{red}{{\cellcolor{gray!45}\textbf{92.2}$_{\pm 0.2}$}}    & 73.4$_{\pm 0.5}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & .007\%                      & 84.7$_{\pm 1.0}$                                    & 84.5$_{\pm 0.8}$                                       & 80.9$_{\pm 1.6}$           & 87.1$_{\pm 0.2}$                                                        & 87.1$_{\pm 0.2}$                                                        & 89.8$_{\pm 0.0}$                                                        & 81.9$_{\pm 1.6}$                                       & {\cellcolor{gray!20}\underline{91.2}$_{\pm 1.9}$}                                         & {\cellcolor{gray!45}\textbf{91.6}$_{\pm 1.2}$}                     & 73.4$_{\pm 0.5}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & .013\%                      & 86.8$_{\pm 0.9}$                                    & 88.6$_{\pm 0.6}$                                       & 87.1$_{\pm 1.2}$           & 90.4$_{\pm 0.0}$                                                        & 90.4$_{\pm 0.0}$                                                        & 89.9$_{\pm 0.1}$                                                        & 80.4$_{\pm 3.4}$                                       & \textcolor{red}{{\cellcolor{gray!20}\underline{91.9}$_{\pm 3.4}$}}                        & \textcolor{red}{{\cellcolor{gray!45}\textbf{92.0}$_{\pm 0.4}$}}    & 79.3$_{\pm 3.0}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & .033\%                      & 87.7$_{\pm 1.4}$                                    & 88.3$_{\pm 1.0}$                                       & 88.6$_{\pm 0.7}$           & {\cellcolor{gray!20}\underline{91.6}$_{\pm 0.2}$}                  & {\cellcolor{gray!20}\underline{91.6}$_{\pm 0.2}$}                  & 90.9$_{\pm 0.1}$                                                        & 89.0$_{\pm 1.2}$                                       & 91.2$_{\pm 4.8}$                                                                               & \textcolor{red}{{\cellcolor{gray!45}\textbf{92.2}$_{\pm 0.2}$}}    & 82.8$_{\pm 1.0}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & .066\%                      & 89.1$_{\pm 0.6}$                                    & 87.9$_{\pm 1.1}$                                       & 88.8$_{\pm 1.0}$           & 91.6$_{\pm 0.2}$                                                        & 91.6$_{\pm 0.2}$                                                        & 91.4$_{\pm 0.2}$                                                        & 86.6$_{\pm 2.1}$                                       & \textcolor{red}{{\cellcolor{gray!45}\textbf{91.9}$_{\pm 2.0}$}}                           & \textcolor{red}{{\cellcolor{gray!20}\underline{91.8}$_{\pm 1.0}$}} & 71.1$_{\pm 0.6}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 & \multirow{-6}{*}{ACM}                                                           & .332\%                      & 89.3$_{\pm 0.9}$                                    & 89.4$_{\pm 0.6}$                                       & 88.7$_{\pm 0.9}$           & {\cellcolor{gray!20}\underline{91.3}$_{\pm 0.2}$}                  & {\cellcolor{gray!20}\underline{91.3}$_{\pm 0.2}$}                  & 91.0$_{\pm 0.5}$                                                        & 89.3$_{\pm 0.6}$                                       & 89.4$_{\pm 0.4}$                                                                               & \textcolor{red}{{\cellcolor{gray!45}\textbf{91.8}$_{\pm 2.3}$}}    & 80.9$_{\pm 2.6}$                                                     & \multirow{-6}{*}{91.7±0.4}                                                \\ \cmidrule(l){2-14} 
\multicolumn{1}{c|}{}                                                 &                                                                                 & .002\%                      & 46.6$_{\pm 2.6}$                                    & 58.9$_{\pm 2.7}$                                       & 54.7$_{\pm 2.6}$           & 61.6$_{\pm 0.7}$                                                        & 56.6$_{\pm 1.1}$                                                        & 71.6$_{\pm 1.8}$                                                        & 71.5$_{\pm 2.2}$                                       & {\cellcolor{gray!20}\underline{77.8}$_{\pm 0.2}$}                                         & \textcolor{red}{{\cellcolor{gray!45}\textbf{81.9}$_{\pm 2.2}$}}    & 72.3$_{\pm 3.1}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & .004\%                      & 57.0$_{\pm 1.4}$                                    & 62.9$_{\pm 0.9}$                                       & 54.9$_{\pm 2.9}$           & 60.4$_{\pm 1.1}$                                                        & 62.0$_{\pm 1.5}$                                                        & 75.4$_{\pm 2.6}$                                                        & 76.2$_{\pm 2.1}$                                       & \textcolor{red}{{\cellcolor{gray!20}\underline{80.9}$_{\pm 1.4}$}}                        & \textcolor{red}{{\cellcolor{gray!45}\textbf{81.7}$_{\pm 3.5}$}}    & 72.3$_{\pm 0.5}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & .007\%                      & 67.5$_{\pm 0.8}$                                    & 61.3$_{\pm 1.6}$                                       & 60.9$_{\pm 0.4}$           & 70.7$_{\pm 0.3}$                                                        & 68.3$_{\pm 0.6}$                                                        & 71.7$_{\pm 4.4}$                                                        & 73.6$_{\pm 0.7}$                                       & \textcolor{red}{{\cellcolor{gray!20}\underline{81.1}$_{\pm 0.6}$}}                        & \textcolor{red}{{\cellcolor{gray!45}\textbf{81.2}$_{\pm 0.4}$}}    & 67.3$_{\pm 1.0}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & .019\%                      & 68.0$_{\pm 1.1}$                                    & 65.7$_{\pm 1.2}$                                       & 64.5$_{\pm 1.1}$           & 73.6$_{\pm 0.2}$                                                        & 73.5$_{\pm 0.4}$                                                        & 76.6$_{\pm 0.6}$                                                        & 74.6$_{\pm 1.1}$                                       & {\cellcolor{gray!20}\underline{77.9}$_{\pm 0.3}$}                                         & \textcolor{red}{{\cellcolor{gray!45}\textbf{80.8}$_{\pm 2.1}$}}    & 72.0$_{\pm 0.9}$                                                     &                                                                           \\
\multicolumn{1}{c|}{}                                                 &                                                                                 & .037\%                      & 67.6$_{\pm 1.5}$                                    & 65.0$_{\pm 1.1}$                                       & 66.6$_{\pm 1.5}$           & 74.6$_{\pm 0.1}$                                                        & 75.2$_{\pm 0.1}$                                                        & 76.9$_{\pm 1.8}$                                                        & 76.4$_{\pm 0.8}$                                       & {\cellcolor{gray!20}\underline{78.5}$_{\pm 0.6}$}                                         & \textcolor{red}{{\cellcolor{gray!45}\textbf{81.9}$_{\pm 3.2}$}}    & 71.6$_{\pm 2.3}$                                                     &                                                                           \\
\multicolumn{1}{c|}{\multirow{-12}{*}{\rotatebox{90}{Heterogeneous}}} & \multirow{-6}{*}{DBLP}                                                          & .186\%                      & 65.7$_{\pm 1.0}$                                    & 66.3$_{\pm 0.8}$                                       & 66.0$_{\pm 1.0}$           & OOM                                                                     & OOM                                                                     & OOM                                                                     & OOM                                                    & OOM                                                                                            & \textcolor{red}{{\cellcolor{gray!45}\textbf{82.1}$_{\pm 0.3}$}}    & {\cellcolor{gray!20}\underline{69.9}$_{\pm 0.9}$}               & \multirow{-6}{*}{80.1±0.9}                                                \\ \bottomrule
\end{tabular}%
}
\end{table}

==> table/methods.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{threeparttable}
\begin{tabular}{cllll}
\multicolumn{1}{l}{Learning Objective}           & Methods & Output &  &  \\
\multirow{10}{*}{Gradient Matching}              & GCond   &        &  &  \\
                                                 & DosCond &        &  &  \\
                                                 & MSGC    &        &  &  \\
                                                 & SGDD    &        &  &  \\
                                                 & FGD     &        &  &  \\
                                                 & GCARe   &        &  &  \\
                                                 & CTRL    &        &  &  \\
                                                 & GroC    &        &  &  \\
                                                 & EXGC    &        &  &  \\
                                                 & MCond   &        &  &  \\
\multirow{4}{*}{Distribution Matching}           & GCDM    &        &  &  \\
                                                 & PUMA    &        &  &  \\
                                                 & CaT     &        &  &  \\
                                                 & FedGKD  &        &  &  \\
\multirow{3}{*}{Kernel Ridge Regression}         & KiDD    &        &  &  \\
                                                 & SFGC    &        &  &  \\
                                                 & GC-SNTK &        &  &  \\
\multicolumn{1}{l}{Eigenbasis Matching}          & GCEM    &        &  &  \\
\multicolumn{1}{l}{Computation Tree Compression} & MIRAGE  &        &  &  \\
\multicolumn{1}{l}{Disentangled Condensation}    & DisCo   &        &  &  \\
\multicolumn{1}{l}{Trajectory Matching}          & GEOM    &        &  & 
\end{tabular}
\end{threeparttable}
\end{table}

==> table/methods_task.tex <==
\newcommand{\cmark}{\ding{51}} % 定义复选框的勾
\newcommand{\xmark}{\ding{55}} % 定义复选框的叉

\begin{table}[]
\centering
\begin{tabular}{clcc}
\hline
Learning Objective                           & Methods & Output & Reproducible \\
\hline
\multirow{10}{*}{Gradient Matching}         & GCond   &        & \cmark       \\
                                             & DosCond &        & \cmark       \\
                                             & MSGC    &        & \cmark       \\
                                             & SGDD    &        & \cmark       \\
                                             & FGD     &        & \cmark       \\
                                             & GCARe   &        & \cmark       \\
                                             & CTRL    &        & \cmark       \\
                                             & GroC    &        & \cmark       \\
                                             & EXGC    &        & \cmark       \\
                                             & MCond   &        & \cmark       \\
\hline
\multirow{4}{*}{Distribution Matching}      & GCDM    &        & \cmark       \\
                                             & PUMA    &        & \cmark       \\
                                             & CaT     &        & \cmark       \\
                                             & FedGKD  &        & \cmark       \\
\hline
\multirow{3}{*}{Kernel Ridge Regression}    & KiDD    &        & \cmark       \\
                                             & SFGC    &        & \cmark       \\
                                             & GC-SNTK &        & \cmark       \\
\hline
Eigenbasis Matching                         & GCEM    &        & \cmark       \\
Computation Tree Compression                & MIRAGE  &        & \cmark       \\
Disentangled Condensation                   & DisCo   &        & \cmark       \\
Trajectory Matching                         & GEOM    &        & \cmark       \\
\hline
\end{tabular}
\caption{Methods and reproducibility}
\label{table:methods}
\end{table}


==> table/notation.tex <==
\begin{table}[htbp]
\vspace{-0.5em}
\label{tab:notation}%
\resizebox{\linewidth}{!}{
  \centering
    \begin{tabular}{cl}
    \toprule
    \textbf{Notations} & \multicolumn{1}{c}{\textbf{Descriptions}} \\
    \midrule
    $\mathbf{DG} = \{ \mathcal{G} \}_{t=1}^{T}$    & Dynamic graph (a set of $T$ discrete graph snapshots) \\
    $\mathcal{G} = (\mathcal{V}, \mathcal{E})$    & Graph with the node set $\mathcal{V}$ and edge set $\mathcal{E}$ \\
    $\mathcal{G}^t = (\mathcal{V}^t, \mathcal{E}^t)$ & Graph snapshot at time $t$ \\
    $\mathbf{X}^{t}$, $\mathbf{A}^t$ & Node features matrix and adjacency matrix of a graph at time $t$ \\
    $\mathbf{x}_v^{t}$, $\mathbf{A}_{(u,v),k}^t$ &  Node features and edge weights of $(u,v)$ under $\mathbf{e}_k$\\
    $\mathcal{G}^{1:t}$, $\mathcal{Y}^{t}$, $\mathbf{G}^{1:t}$, $\mathbf{Y}^{t}$ & Graph trajectory, labels and their corresponding random variables \\
    $\mathbf{e}$, $\mathbf{e}_i$, $\mathbf{E}$ & Latent environments and their support\\
    $\mathbf{z}_{v,k}^{t}$, $\mathbf{z}_{v}^{\mathbf{e},t}$, $\mathbf{z}_{v}^{\mathbf{e}}$ & Node representations under $\mathbf{e}_k$, at time $t$ and at overall time slices\\
    $\mathbf{z}$, $\mathbf{y}$ & Observed environment sample with its label\\
    $d$, $d^{\prime}$ & Dimension for $\mathbf{x}_v^t$ and $\mathbf{z}_{v,k}^t$, respectively\\
    $K$ & Number of underlying environments (number of convolution channel)\\
    $f(\cdot)$, $w(\cdot)$, $g(\cdot)$ & Model, encoder, and the link predictor\\
    $\ell(\cdot)$ & The loss function\\
    $q_\phi$, $p_\omega$ & The prior distribution and variational distribution of environments\\
    $\mathbb{I}^\star(\cdot)$, $\mathbb{I}(\cdot)$ & Invariant pattern recognition function and its implementation\\
    $\mathcal{P}_\mathbf{e}^I$, $\mathcal{P}_\mathbf{e}^V$, $\mathcal{P}_\mathbf{e}^I(v)$, $\mathcal{P}_\mathbf{e}^V(v)$ & Summary of spatio-temporal invariant/variant patterns for each node\\ 
    $\mathbf{Z}^{1:t}$, $\mathbf{Z}_{\mathcal{P}_\mathbf{e}^I}^{1:t}$, $\mathbf{Z}_{\mathcal{P}_\mathbf{e}^V}^{1:t}$ & Summary of node representations, and their variants under  $\mathcal{P}_\mathbf{e}^I$ and $\mathcal{P}_\mathbf{e}^V$\\
    $\mathcal{S}_{\mathrm{ob}}$, $\mathcal{S}_{\mathrm{ge}}$ & Observed and generated environments sample libraries \\
    $s$, $\mathbf{s}_v$ & Intervention samples from $\mathcal{S}_{\mathrm{ob}}\cup\mathcal{S}_{\mathrm{ge}}$ and their summary for node $v$\\
    $\mathrm{do}(\cdot)$ & $do$-caculus for causal interventions\\
    $\mathcal{L}_\mathrm{task}$, $\mathcal{L}_\mathrm{risk}$, $\mathcal{L}_\mathrm{ECVAE}$ & Task loss, the invariance loss and the ECVAE loss\\
    $\alpha$, $\beta$ & Hyperparameters for loss trade-off\\
    
    \bottomrule
    \end{tabular}%
}
\vspace{-1em}
\end{table}%


==> tasks.tex <==
\newpage
\section{Tasks}

\subsection{Basic methods}:
\begin{itemize}
    \item 
\end{itemize}
\include{table/methods_task}

\subsection{Datasets}:
\todo{zy}
\begin{itemize}
    \item 
\end{itemize}
\subsection{Tasks}
\begin{itemize}
  \item Different compression ratios
  \item Transferability across architectures
    \begin{itemize}
        \item + graph transformer
    \end{itemize}
  \item NAS
  \item Structures (generate new datasets)
\end{itemize}

\newpage

